Evaluating Open-Domain Dialogues in Latent Space with Next Sentence Prediction and Mutual Information

The long-standing one-to-many issue of the open-domain dialogues poses significant challenges for automatic evaluation methods, i.e., there may be multiple suitable responses which differ in semantics for a given conversational context. To tackle this challenge, we propose a novel learning-based automatic evaluation metric (CMN), which can robustly evaluate open-domain dialogues by augmenting Conditional Variational Autoencoders (CVAEs) with a Next Sentence Prediction (NSP) objective and employing Mutual Information (MI) to model the semantic similarity of text in the latent space. Experimental results on two open-domain dialogue datasets demonstrate the superiority of our method compared with a wide range of baselines, especially in handling responses which are distant to the golden reference responses in semantics.

==> Tab/IAA.tex <==

% \begin{table*}[!hbt]
% \centering
% \scalebox{1}{
% \begin{tabular}{c|ccc|ccc} 
% % \cline{1-5}
% \toprule
% IAA & \multicolumn{3}{c|}{DailyDialog} & \multicolumn{3}{c}{PersonaChat} \\
% \midrule
% % \cline{1-5}
%  & Annotator1 & Annotator2 & Annotator3 & Annotator1 & Annotator2 & Annotator3 &
%  \midrule
% Annotator1       &- &0.6896 & 0.6035 & - &0.4496 & 0.5547 \\
% Annotator2     &0.6896 & - & 0.6434 &0.4496 &- &0.6315 \\
% % Annotator3     & 0.6035 & 0.6434 & - & &  &  

% \bottomrule
% \end{tabular}
% }
% \caption{Inter-Annotator agreement (IAA)}\label{tab:IAA}
% \end{table*}

% \begin{table}[!h]
% \scalebox{0.8}{
% \begin{tabular}{c|ccc} 
% % \cline{1-5}
% \toprule
%  \multicolumn{4}{c}{DailyDialog} \\
% \midrule
% % \cline{1-5}
%  \textbf{Annotator} & \multicolumn{3}{c}{Cohen's Kappa} &
%  \midrule
%  & Annotator1 & Annotator2 & Annotator3 &
%  \midrule
% Annotator1       &- &0.6896 & 0.6035&
% \midrule
% Annotator2     &0.6896 & - & 0.6434 & 
% \midrule
% Annotator3     & 0.6035 & 0.6434 & - &
% \bottomrule
% \end{tabular}
% }
% \caption{Inter-Annotator agreement (IAA)}\label{tab:IAA1}
% \end{table}


% \begin{table}[!h]
% \scalebox{0.8}{
% \begin{tabular}{c|ccc} 
% % \cline{1-5}
% \toprule
%   \multicolumn{4}{c}{PersonaChat} \\
% \midrule
% % \cline{1-5}
%   \textbf{Annotator} & Annotator1 & Annotator2 & Annotator3 &
%  \midrule
% Annotator1      & - &0.4496 & 0.5547& \midrule
% Annotator2     &0.4496 &- &0.6315 & \midrule
% Annotator3     & 0.5547 & 0.6315 & - &  
% \bottomrule
% \end{tabular}
% }
% \caption{Inter-Annotator agreement (IAA)}\label{tab:IAA2}
% \end{table}
%----------------------------
% \begin{table}[]
% \begin{tabular}{|c|ccc}
% \hline
%                       & \multicolumn{3}{c|}{DailyDialog}                                         \\ \hline
% annotator              & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{3} \\ \hline
% 1                      & -                      & 0.6896                 & 0.6035                 \\ \hline
% 2                      & 0.6896                 & -                      & 0.6434                 \\ \hline
% 3                      & 0.6035                 & 0.6434                 & -                      \\ \hline
% \multicolumn{1}{|l|}{} & \multicolumn{3}{c}{PersonaChat}                                          \\ \hline
% 1                      & -                      & 0.4496                 & 0.5547                 \\ \hline
% 2                      & 0.4496                 & -                      & 0.6315                 \\ \hline
% 3                      & 0.5547                 & 0.6315                 & -                      \\ \hline
% \end{tabular}
% \caption{Inter-Annotator agreement (IAA)}\label{tab:IAA2}
% \end{table}
%----------------------------
\begin{table}[!h]
\centering
\scalebox{0.9}{

\begin{tabular}{c|ccc} 
% \cline{1-5}
\toprule[2pt]
 \multicolumn{4}{c}{DailyDialog} \\
\midrule
% \cline{1-5}
 \multicolumn{1}{l}{\textbf{Annotator}} & \multicolumn{3}{c}{Cohen's Kappa} 
 \midrule
  \multicolumn{1}{l}{} & Annotator1 & Annotator2 & Annotator3 
 \midrule
 \multicolumn{1}{l}{Annotator1}       &- &0.6896 & 0.6035
\midrule
 \multicolumn{1}{l}{Annotator2}      &0.6896 & - & 0.6434 
\midrule
 \multicolumn{1}{l}{Annotator3}      & 0.6035 & 0.6434 & - 
% \bottomrule[2pt]
\toprule[2pt]
% \cline{1-5}
  \multicolumn{4}{c}{PersonaChat} \\
\midrule
% \cline{1-5}
  \multicolumn{1}{l}{\textbf{Annotator}} & Annotator1 & Annotator2 & Annotator3 
 \midrule
 \multicolumn{1}{l}{Annotator1}      & - &0.4496 & 0.5547 \midrule
 \multicolumn{1}{l}{Annotator2}     &0.4496 &- &0.6315  \midrule
 \multicolumn{1}{l}{Annotator3}      & 0.5547 & 0.6315 & - 
\bottomrule[2pt]
\end{tabular}
}
\caption{Inter-Annotator agreement (IAA)}
\label{tab:IAA}
\end{table}

==> backup.tex <==


\begin{abstract}
% The one-to-many problem of open domain dialogue causes significant challenges for the designing of automatic evaluation metrics. Recent efforts attempt to solve it by comparing the similarity of generated response with the conversational context. Although some studies achieve promising results by designing discriminative models learning from multiple responses directly or in latent space, their method is lack of interpretability due to the nature of neural network and cannot be applied widely as the multiple responses is unavailable in most existing dataset.
% Therefore, we propose a latent space-based, information theoretic guided dialogue evaluation method, which can capture implicit correct responses and enhance the interpretability of the evaluation by incorporating information theory. 
% The experiment results and analysis confirm our method achieves best overall performances on Pearson and Spearman correlations with human annotation, and handle the one-to-many issue .
%Evaluating the generated text is essential for many NLG tasks, especially open-domain dialogue.
The long-standing one-to-many issue of the open-domain dialogues poses significant challenges for automatic evaluation methods, i.e., a conversational context might have multiple reasonable responses which differ from each other in semantics. 
%Inspired by information theory and Conditional Variational Autoencoders (\textbf{C}VAEs), 
To tackle this challenge, we propose a novel learning-based automatic evaluation metric (\textbf{CMN}), which can robustly evaluate open-domain dialogues by augmenting Conditional Variational Autoencoders (\textbf{C}VAEs) with the Next Sentence Prediction (\textbf{N}SP) objective and employing Mutual Information (\textbf{M}I) to model the semantic similarity of text in the latent space.  
%in the training phase, which strengthen the model's ability to identify the correct context-reference pair and the sentence order information.
% we propose a novel open-domain dialogue evaluation metric (\textbf{CMN}) which combines Mutual Information (\textbf{MI}) and CVAEs strengthened by Next Sentence Prediction (\textbf{NSP}) task. This metric is then used to 
% %measure the semantic similarity of generated response with reference response, and its conversational context. 
% evaluate whether a response candidate is reasonable to its conversational context.
Experimental results on two open-domain dialogue datasets demonstrate the superiority of our method compared with a wide range of baselines, especially in handling responses which are distant to the references in semantics. 

%the one-to-many nature  open-domain dialogue
% In addition, we also provide a detailed analysis of our method's %performance on selected multi-diversity datasets to confirm the 
% effectiveness in handling the one-to-many nature in the open-domain dialogue.


% multi-diversity datasets and lower-diversity datasets demonstrate the high quality of our evaluation metrics.
\end{abstract}

\section{Introduction}

% 1. Introduce the context and background of your research topic
%one-to-many, human annotation, less inpretability
% 2. What will the work of this paper achieve, i.e., the outcome of this paper?
%incorporating mi and vae in dialogue evalutation field, to best known, which is the first attempt. solving the one-to-many nature to some extent
% 3. What is the significance of the work proposed in this paper? i.e., what will it allow us to do what we can’t do now and who wants to do that?
%one-to-many nature, allowing the evaluation of potential response which is less similar to context in semantic.
%Extend the application of Mutual Information, combaining Information theory and VAE to evaluate open-domain dialogue.
%Few previous work combing the Information theory and generative model for evaluation
%We further extend the Mutual Information application, applying it in NLG evaluation
%avoid human annotation in training phase

% 4.Summarise the proposed approach of the paper
%method, vae and MI, MI lower bound approximation,  model architecture 
% 5.Summarise the contributions of the paper
% Information theory and VAE to evaluate open-domain dialogue.
% Few previous work combing the Information theory and generative model for evaluation
% Extend the application of Mutual Information
% We further extend the Mutual Information application, applying it in NLG evaluation
% Considering One-to-many issue

% In recent years, with the rapid development of deep learning, open-domain dialogue generation has made great progress~\cite{Chen2021ReasoningID, Hu2019GSNAG, Wolf2019TransferTransfoAT, Chan2019ModelingPI, Qiu2019AreTS}. The automatic evaluation metric is significant for the  Natural Language Generation (NLG) tasks~\cite{Dathathri2020PlugAP, Gu2019LevenshteinT}. \textcolor{orange}{However, there is still no widely accepted evaluation metrics can perform well in evaluating open-domain
% generative dialogue systems because of the diversity of languages }~\cite{Gatt2018SurveyOT}. Therefore, how to evaluate the quality of generated text becomes an urgent problem to be solved in open domain dialogue. 
% Many automatic evaluation metrics have been proposed to evaluate the open domain dialogue system. 

Open-domain dialogue generation is a prominent research direction in conversational AI due to the variety of useful applications, e.g., personal digital assistants and customer service~\cite{huang_challenges_2019}. While evaluating natural language generation (NLG) systems is notoriously difficult, the evaluation of the open-domain dialogue generation introduces an extra layer of complexity, as a variety of responses can be generated, each valid in its own context, yet semantically very different~\cite{li_diversity-promoting_2016, Gu2019DialogWAEMR, qiu_are_2019}. 
For example, given the conversational context ``\textit{Iverson is my all time favourite player.}'', responses such as ``\textit{He is my favourite player too.}'' or  ``\textit{Yes, his quickness is amazing!}'' are both contextually relevant but semantically different. 
%\textcolor{red}{[CL: perhaps show a concrete examples here for the one-to-many issue.]}

% This also makes 
% More importantly, how to measure the controllability of the generated text remains an open question
% [say something about what is a good response in a dialogue setting]. 

%Evaluating natural language generation (NLG) systems is notoriously complex: the same input can be expressed in a variety of output texts, each valid in its own context, making evaluation with automatic metrics far more challenging than in other NLP contexts

Existing approaches for evaluating open-domain dialogue systems can be broadly divided into two different categories: reference-based and reference-free metrics. The reference-based metrics typically score a system by computing how similar its output response is to the \textit{gold-standard} reference. Popular metrics under this category either rely on surface-form similarity by counting the $n$-gram overlap between the response candidate and the reference (e.g., BLEU~\cite{papineni_bleu_2002}, ROUGE~\cite{lin_rouge_2004}, and METEOR~\cite{banerjee_meteor_2005}), or by calculating the similarity based on high-dimensional representations learned for the response and the reference such as BERTScore~\cite{Zhang2020BERTScoreET}. One noticeable limitation of reference-based metrics is that they are reference centric and do not take the context of the conversation into consideration. However, due to the well-known one-to-many issue in the open-domain dialogue~\cite{li_diversity-promoting_2016, Gu2019DialogWAEMR, qiu_are_2019}, a good response that matches well to its context could express significantly different semantics to its reference, thus only comparing the similarity between the reference and the generated response is inadequate. 
%The first way measures the semantic similarity by comparing sentence word overlap or the embedding of the reference and response candidate, like BLEU~\cite{papineni_bleu_2002}, METEOR~\cite{banerjee_meteor_2005} and ROUGE~\cite{lin_rouge_2004}, which calculate the word overlap while BERTScore~\cite{Zhang2020BERTScoreET} and BLEURT~\cite{Sellam2020BLEURTLR} consider the word embedding similarity.
%and PONE~\cite{Lan2020PONEAN} designing a discriminative model . 

To tackle the one-to-many issue, some other works~\cite{Tao2018RUBERAU, Sinha2020LearningAU, Ghazarian2019BetterAE, zhao_designing_2020} proposed reference-free metrics to evaluate the generated response by measuring its similarity with the corresponding conversational context, by designing discriminative models trained on the context and the reference to judge whether the generated response matches the context well. As these discriminative metrics are typically trained using a single relevant (i.e., positive) response and multiple negative samples, \citet{sai_improving_2020} argued that such metrics should be trained with multiple relevant and irrelevant responses for any given context to allow for robust evaluation. 
However, most existing datasets do not contain multiple relevant responses as references, making this recommendation impractical. 

%argue EMS's assumption: limitation of prior
\citet{chan_enhancing_2021} took a different approach to evaluate the generated response in the latent space produced by CVAEs, as it can encode discrete text data into a smooth latent space. Specifically, they proposed to use the prior distribution to approximate the conditional distribution for all the feasible responses to tackle the one-to-many issue with limited data. However, as they only use a single response for training, there is no guarantee that the prior distribution can represent a rich set of feasible responses~\cite{Li2019ASE}. 
%as the datasets only have a single response and the prior distribution of the model trained on it is hard to approximate all latent reasonable responses~\cite{Li2019ASE}.
%the corresponding representation only close to such that which is semantically similar to the given response in the smooth latent space %\textcolor{red}{[provide some reasons]}.
%that neither theoretical or empirically 
%where latent representations of similar sentences should be close to each other and vice versa~\cite{Li2019ASE}. 
%However, their prior distribution does not contain enough latent response information, although they declared it can be regarded as the substitute set of all reasonable ground-truth references.
%discourse 
Nevertheless, few prior works seek to model the intra-relation between a context and a response through the next sentence prediction (NSP) task directly, which can provide a strong signal for indicating the sequential dependencies between the context and response.
%modelled by a good fit for discourse relation recognition


% More importantly, there is no theoretical guarantee behind both previous reference-based, and reference-free metrics, and these metrics only calculate the context-response or reference-response semantic similarity. 
% Meanwhile, semantics can be regarded as latent variables and thus it is feasible to introduce Mutual Information (MI) to measure semantic dependence between variables in latent space produced by VAE. 
% As a result, we can utilize MI in latent space to calculate the dependence between response candidates and feasible references to acquire a more accurate evaluation score.

% By comparing the semantic similarity of conversational context with response in a smooth latent space produced by VAE model, they can tackle the one-to-many issue of open dialogue evaluation.
%However, their prior distribution does not contain enough latent response information, although they declared it can be regarded as the substitute set of all reasonable ground-truth references.
%However, during the training phase of EMS, they only encode one context-reference pair and lack the information of all reasonable references. 
%segmentation %limitation of the prior distribution
%Another shortcoming of EMS is that it does not take the order information between conversational context and reference into account. %as there is lack of obvious segmentation markers between them. 
%eva method
%More importantly, there is no theoretical guarantee behind both previous reference-based, and reference-free metrics, and these metrics only calculate the context-response or reference-response semantic similarity. 
% evaluation phase and detailed enough evaluation analysis for solving the one-to-many issue of open dialogue evaluation. 
%introduce MI
%Meanwhile, semantic can be regarded as latent variables, so it is feasible to introduce MI into evaluation metrics. 
%Therefore, even there is only one relevant reference in most existing datasets, we can obtain the distribution of a series of similar references in the latent space, which helps solve the one-to-many problem in the open-domain dialogue system to a great extent. 
% Meanwhile, semantics can be regarded as latent variables and thus it is feasible to introduce Mutual Information (MI) to measure semantic dependence between variables in latent space produced by VAE. 
% As a result, we can utilize MI in latent space to calculate the dependence between response candidates and feasible references to acquire a more accurate evaluation score.
%\textcolor{red}{[CL: can you add some text to explain why calculating MI in the latent space is desired, rather than, say with raw text or embedding? What is the key benefits of operating in the latent space?]}
% But we consider compute both pair-wise semantic similarities via Mutual Information (MI), a fundamental concept in information theory, measuring the dependence between two random variables.
%The advantage of using InfoNCE includes not only providing theoretical guarantee for measuring sentence similarity, but also introducing comprehensive information by contrastive learning during the evaluation process.

To tackle the one-to-many issue, we design a novel learning-based automatic evaluation metric (\textbf{CMN}), which can robustly evaluate open-domain dialogues \textit{without} requiring multiple gold-standard references. Our method consists of a training stage and an evaluation stage. In the training stage, the \textbf{C}VAEs is augmented with a Next Sentence Prediction (\textbf{N}SP) objective~\cite{Devlin2019BERTPO}, which plays a crucial role in addressing the one-to-many issue in dialogue evaluation, especially when the semantics of the generated response are distant from the reference but still relate well to the context. 
%and employs Mutual Information (\textbf{M}I) to model the semantic similarity of both the context to response and reference to response pairs simultaneously. 
%Such a design strengthens our model's ability to capture the sequential dependencies between the context and response, as well as leverage the information from references.
%identify the correct context-reference pair and the sentence order information.

% In the training phase, we utilise CVAE to encode the dialogue into the latent space and augment CVAE with the NSP objective in BERT~\cite{Devlin2019BERTPO} in order to strengthen the model's discriminative ability \textcolor{orange}{of context and reference pair and sentence order information.} 
%The NSP objective. NSP evaluates whether the response is the next reasonable reply to the context in this situation. 
In the evaluation phase, we score a response candidate by calculating the Mutual Information (\textbf{M}I) of the context-response and response-reference pairs in the latent space, which are then combined through a weighting controlled by the NSP probability.
%by calculating the MI and the NSP score of the context-response and the MI response-reference pairs in the latent space. 
However, it is intractable to calculate MI directly as we only have access to samples instead of the prior and posterior distributions~\cite{mcallester_formal_2018, paninski_estimation_2003}. 
% \textcolor{blue}{[the latent variables]}
To tackle this challenge, we propose to employ a contrastive learning method based on Noise Contrastive Estimation (NCE)~\cite{Gutmann2012NoiseContrastiveEO,logeswaran_content_2018} to calculate the lower bound of MI.
Overall, introducing the NSP objective and mutual information strengthens our model's ability to capture the sequential dependencies between the context and response, as well as to leverage the information from references.
%, which can result in better representation of the context-response and the reference-response pairs.
% which can bring the model the comprehensive semantic information of context-response and reference-response pairs and provide theoretical guarantee at the same time.
%systematically fusion information of NSP and MI??
%we utilise InfoNCE to calculate the lower bound of MI between latent variables containing dialogue sentence information.

%latent variables of the context, response candidate, and gold reference, which are encoded in 
%as well as between the gold reference and the response candidate in the latent space. 



%Unlike EMS, we introduce the Next Sentence Prediction (NSP) task in BERT~\cite{Devlin2019BERTPO} in training phase to infer the relationship between sentences. The NSP task enables the CVAEs model to discriminate which context-response pair is mismatched via randomly replacing the training reference by a certain percentage. Therefore, the posterior and prior distributions of CVAE model will contain more precise potential reasonable response information and sentences sequential information, 
%Besides, the Segment Embedding of NSP task allows the posterior and prior distribution of CVAE can contain the sequential information of sentences as well. 

% Mutual Information (MI) 
% MI has been widely used in lots of fields and thus can provide theoretical guarantee, and increase the interpretability of evaluation stage as well. 
% %To our best known, it is the first attempt to combine MI and CVAE in automatic open dialogue evaluation field. 
% Meanwhile, semantic can be regarded as latent variables, therefore it is feasible to utilize InfoNCE to estimate MI in latent space produced by CVAE. When utilizing utilize InfoNCE, the model can capture comprehensive information from both context and reference perspectives via contrastive learning from negative samples.

Experimental results on two open-domain dialogue datasets show the superiority of our method compared to a wide range of baseline metrics based on both Pearson and Spearman correlations with human annotations. In addition, we provide a detailed analysis of the effectiveness of our proposed method in solving the one-to-many issue in open-domain dialogue evaluation. 
Our code and data will be made available.
%on semantic similar and diverse selected dialogue pairs. 

% Our contributions can be summarised as follows: (1) we propose a novel automatic evaluation metric (CMN), which combines NSP incorporated CVAEs and MI; %(2) our metric incorporate the NSP task to strengthen the prior and posterior distribution of CVAEs; 
% %in terms of discriminating mismatched sentence pair and internal order; 
% (2) we extend the application of MI. To the best of our knowledge, this is the first attempt to apply MI in the automatic evaluation metric field; and (3) we provide a detailed analysis of how effective our method is in dealing with the one-to-many nature of open-domain dialogue evaluation, especially when the response relates well with its context but is far away from the gold reference in semantics. Our code and data will be made available.

% As for Variational AutoEncoder (VAE) and Conditional Variational AutoEncoder (CVAE), especially the text-VAE~\cite{Bowman2016GeneratingSF}, semantic information can be regarded as a latent variable. 
%From these previous studies, both reference-based metrics and reference-free metrics calculate the semantic similarity between the generated text and the context or ground-truth reference. As for Variational AutoEncoder(VAE), especially the text-VAE~\cite{Bowman2016GeneratingSF}, semantic information can be regarded as a latent variable. \cite{Chan2021EnhancingTO} first introduced VAE into the field of automatic evaluation metrics, designing an automatic evaluation system called EMS. By comparing the semantic similarity of conversational context with response in a learned smooth latent space, they can tackle the one-to-many issue in dialogue system evaluation. However, there is no theoretical guarantee behind their method and there is no evaluation detail. Mutual Information (MI) is a key concept in information theory, measuring the dependence between two random variables. As a result, incorporating MI and VAE is a feasible method in the field of automatic evaluation metrics. Moreover, as one important theory in information theory, MI can also provide theoretical support for designing automatic evaluation metrics and increase the interpretability. Another disadvantage of EMS is that the input x and r of the encoder do not have obvious segmentation markers, but directly combine $x$ and $r$ into the encoder may cause not enable the encoder to recognize the segment of sentence pairs, resulting in suboptimal performance.



% Our method can be divided into two phases: training phase and evaluation phase. In the training phase, we initially utilize CVAE to map the dialogue sentence into a latent (or semantic) space and introduce NSP task to strengthen the model's discriminative ability of context and reference pair and sentence order information. When the input of the encoder is a positive sample, the NSP loss is regarded as an additional loss to CVAE's loss. Otherwise, the model is trained as a normal CVAE. In the evaluation phase, InfoNCE to estimate the MI between latent variables containing context or response information.
%MI part

%not clear
% The posterior distribution %$q(z|c,r)$ 
% obtained from the negative sample does not have the conditions for sampling from it and sending it to the decoder, nor does it have the conditions for approximating the prior distribution. Therefore, in order to solve this problem, considering the generation process after the training of VAE, we decide to sample latent variables from the conditional prior distribution %$p(z|c)$  %$p(z|x)$ $ q(z|c,x)$
% of VAE as the hidden variable of the decoder, which can also make prior distribution be closer to posterior distribution, resulting in better results than EMS. 






%related work
\section{Related Works}

% To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

%\subsection{Evaluation Metrics}
%Existing evaluation metrics could be divided into two types, reference-based metrics and reference-free metrics.

%\subsection{Evaluation Metrics}
\noindent\textbf{Reference-based metrics.}~~The reference-based metrics mainly compare the semantic similarity between a ground-truth reference and a generated response. 
Representative metrics that calculate word overlap include BLEU~\cite{papineni_bleu_2002}, METEOR~\cite{banerjee_meteor_2005} and ROUGE~\cite{lin_rouge_2004}. %Existing metrics calculating the word overlap include
% However, they are weakly related to human judgement.

Unlike these metrics comparing the word overlap directly, embedding metrics first convert sentences into a high dimensional representation and calculate the semantic similarity between them. With the development of large-scale pre-training models, some embedding metrics such as BERTScore~\cite{Zhang2020BERTScoreET} and BLEURT~\cite{Sellam2020BLEURTLR} enhance the sentence representation via large-scale pre-training models. 
However, these automatic reference-based metrics cannot deal with the well-known one-to-many problem in the open-domain dialogue.
%BERTScore shows strong system and segment level correlation with human score by leveraging the pre-trained contextual embedding from BERT models and matches words in candidate and reference sentences by cosine similarity. \textcolor{red}{[CL: can you say a bit more the benefit of methods like BERTScore?]}

%PONE~\cite{Lan2020PONEAN}. 



\noindent\textbf{Reference-free metrics.}~~Existing reference-free metrics attempt to design discriminative models to solve the one-to-many issue by calculating the similarity between the context and the response candidate.
% where the recent representative work include RUBER~\cite{Tao2018RUBERAU}, MAUDE~\cite{sinha_learning_2020} and EMS~\cite{chan_enhancing_2021}.
RUBER~\cite{Tao2018RUBERAU} is an unsupervised metric calculating the similarity of the generated response with both the context and the response. MAUDE~\cite{Sinha2020LearningAU} employs a large-scale pre-trained model to convert sentences into hidden representations and leverage the temporal transitions between them.
\citet{sai_improving_2020} argued that such models should be trained on datasets containing multiple responses. However, most existing datasets only contain a single relevant reference. To solve this issue, EMS~\cite{chan_enhancing_2021} first attempted to utilise the CVAEs to learn the reference information with limited data and approximate all feasible responses with the prior distribution. However, their model's prior distribution and sampled variables do not necessarily contain all the feasible response information for a given context, as EMS is only trained with a single reference. We consider combining reference-based and reference-free methods by augmenting the CVAEs with the NSP objective and employing MI to evaluate the response candidates.
% Specifically, they denoted that $r_i$ is a reasonable response of a given context $x$, and $\{r_k\}_{k=1}^N$ is the set containing all feasible responses context $x$. The prior distribution $P(z|c)$ conditioned on conversational context $c$ can capture the information of any reasonable latent response 
% %to some extent after the process of approximation the posterior distribution of 
% %CVAE, 
% and the latent variables $z$ sampled from the prior distribution can contain information of any feasible latent response $r_i$. 
 %In addition, 
% The EMS model \textcolor{orange}{cannot discriminate} whether the input context-response pair is matched and \textcolor{orange}{learn the order information} of the sentence pair during the training process, which causes the prior distribution and the latent variables sampled from it to lack precise latent reference information and sequential sentence information.

% Recent studies focus on reference-free metrics to solve the one-to-many nature. They compare the semantic similarity between context and response candidates by designing machine learning models to judge the relationship between them.
% Recent learning-based reference-free metrics include RUBER~\cite{Tao2018RUBERAU}, MAUDE~\cite{sinha_learning_2020} and EMS~\cite{Chan2021EnhancingTO}. However, these metrics lack the perspective of ground-truth response and require human-annotated data to train the model. In addition, there is no theoretical guarantee behind their similarity measurement. EMS first evaluated open dialogue by computing the context-response similarity in latent space, but it has the following shortcomings: 
% %The encoder of EMS did not take the sequence relationship and correctness of sentence pair into account; 
% The prior distribution of EMS lacks enough reference information to approximate all reasonable references; There is no explicit theoretical guarantee for its evaluation stage, and they did not provide enough analysis of the effectiveness in solving one-to-many nature.
% We propose a new evaluation method that includes reference and reference-free perspectives information by extending the application of MI in the open domain dialogue evaluation field and combining it with CVAE. Meanwhile, we incorporate the NSP task into the CVAE model to strengthen it.% in terms of discriminating mismatched sentence pair and internal order. 


% \subsection{Mutual Information}
% Mutual Information usually measures the dependence between two random variables and has been widely applied to a series of tasks in deep learning, including the information bottleneck~\cite{https://doi.org/10.48550/arxiv.physics/0004057}, generative modelling~\cite{Chen2021ReasoningID} and representation learning~\cite{gholami2018unsupervised}.
% %, there are few previous studies applied it into automatic open domain dialogue evaluation field.
% Given two random variables A and B, mutual information can be regarded as how much information about B is contained in A, and vice versa. Therefore, the mutual information between A and B can be expressed by the following formula:

% \begin{equation}
%     \begin{aligned}
%           I(A,B) &= H(A) - H(A|B) \\
%                  &= H(B) - H(B|A)
%     \end{aligned}
% \end{equation}
% where $H$ is the entropy.
% % In natural language processing, variables A and B can be regarded as different sentences, such as conversational context and response. 
% Considering a function $f$, which takes $A$ and $B$ as its input, then the goal of is to learn parameters of the function $f$ that maximizes $I(A,B)$.

% % However, MI is intractable when $f$ contains modern encoders, like neural network~\cite{Paninski2003EstimationOE}, thus we need to resort to calculate the lower bound of $I(A,B)$. %We use

% \noindent\textbf{InfoNCE}~~As in most cases, the MI is intractable~\cite{Paninski2003EstimationOE}, InfoNCE~\cite{Logeswaran2018AnEF, Oord2018RepresentationLW,Kong2020AMI} is to estimate the mutual information lower bound 
% % and have been shown to work well
% , which is based on Noise Contrastive Estimation(NCE)~\cite{Gutmann2012NoiseContrastiveEO}, the formula is:

% \begin{equation}
%     \begin{aligned}
%           &I(A,B) \geq E_{p(A,B)}[f_{\theta}(a,b) \\
%           &-E_{q(\hat{B})}[log \sum_{\hat{b} \in \hat{B}} \text{exp} f_{\theta}(a, \hat{b})]] + log|\hat{B}|
%     \end{aligned}
% \end{equation}
% where $E$ is the expectation, $a$ and $b$ are two random variables, $f_{\theta}(a,b)$ is a function parameterized by $\theta$, and $\hat{B}$ is a set containing samples drawn from a proposal distribution $q(\hat{B})$. The set $\hat{B}$ consists of one positive sample $b$ and $|\hat{B}|$ - 1 negative samples.


\section{Methodology}

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.89\textwidth]{model.pdf}
  \caption{The architecture of the proposed model. The left part is the training phase, containing two encoders to represent the context-response pair and context. The NSP task is incorporated after the encoding of the context and response pair. The right part is the evaluation phase, in which the generated text is the response candidate and will be evaluated via the MI method during this stage. The Segment Embeddings are used for the NSP task.} 
  %The dotted box represents the first Encoder in the training phase is used to convert the sentence pairs twice in the evaluation phase.}
  \label{fig: Model}
\end{figure*}


% This is achieved by augmenting CVAE with a Next Sentence Prediction (NSP) objective and employing Mutual Information (MI) to model the semantic similarity of both context to response and reference to response simultaneously.
% propose an automatic dialogue evaluation metric by combining strengthened CVAE and MI, containing training and evaluating phases as illustrated in Figure~\ref{fig: Model}.
%%TODO more detail about training and evaluation process


%limitation of prior dis: limited input, unable to discriminate negative samples,
%necessity of NSP: regularize the training phase, 
% Our motivation comes from information theory.


% The NSP task enables the CVAE model to discriminate which context and response pair is mismatched via randomly replacing the training reference by a certain percentage when feeding the sentence pair to model. Thus the posterior and prior distributions of CVAE model will contain more precise potential reasonable response information, as the latter will only approximate the former when the input sentence pair is unchanged during the CVAE's training process. Besides, the Segment Embedding of NSP task allows the posterior and prior distribution of CVAE can contain the sequential information of sentences as well


%Besides, there are no theoretical guarantee behind EMS and other learning-based evaluation metrics as most of them use neural network based methods to estimate the semantic similarity between sentences 


\subsection{Overall Architecture}

In this section, we describe the proposed automatic evaluation metric, CMN, in detail. As shown in Figure~\ref{fig: Model}, the overall architecture of CMN consists of two stages: training and evaluation.   
The primary purpose of the training stage is to capture the dialogue information in the latent space, which is strengthened by incorporating the NSP objective into the CVAE model. 
%Specifically, we use two encoders to convert context-reference pairs and context into latent semantic space. When encoding the context-reference pair, we introduce the NSP task to strengthen the model's ability. 
%The evaluation phase is to evaluate response candidates with their context by calculating the MI and the NSP probability between them and the MI between the reference and the response candidates as well.
The evaluation stage is to evaluate the response candidates by calculating the MI of the context-response and response-reference pairs in the latent space, which are then combined through a weighting by the NSP probability of the response candidate.
%with their contexts by calculating the NSP probability and the MI between them, as well as the MI between the references and response candidates.

%We first use the same encoder part of the CVAEs model in the training phase to get the distributions containing the latent semantic information of the context-reference pair, the context-response pair, and the context, respectively. We then conduct sampling from each distribution and perform the InfoNCE method to compute the semantic dependency. It is noticeable that the NSP task is also included when encoding the context-response pair, and the probability is considered when computing the final matching score.
\subsection{Training Stage}
% In the training phase, we utilize two Bert encoders, one is for encoding context and response sentence pair into $h_q$, the other is for encoding context sentence into $h_p$. Then $h_q$ and $h_p$ will be used to approximate the posterior and the prior distributions of CVAE, respectively.


%\textcolor{red}{[CL todo: some motivation text here.]}
The training process of our proposed method is illustrated in the left part of Figure \ref{fig: Model}. We employ two BERT encoders: the first is used to encode the context-reference pairs, and the second encodes the context only.
% and produce $p(z|h_p)$ to estimate the prior distribution $p(z|c)$. 
%Both two encoders utilize Bert pre-trained model. First, we need to transfer the sequence into the vector, as we all know, 
Formally, the encoding process is: 
% % \begin{equation}
%     \begin{align}
%           h_c &= emb_c + pos_c + seg_c \nonumber\\
%           h_r &= emb_r + pos_r + seg_r
%     \end{align}
% % \end{equation}
% where $emb_c$ is the word embedding of context, $emb_r$ is the word embedding of context, $pos_c$ and $pos_r$ are the position embedding and  $seg_c$ and $seg_r$ are Segment embedding of NSP task.
% Then we feed $h_c$ and $h_r$ into \textcolor{red}{Bert} encoder to produce $q(z|h_q)$ and $p(z|h_p)$, then utilize them to approximate posterior distribution $q(z|c,r)$ and the posterior $q(z|c)$, respectively. We assume that $q(z|c,r)$ and $p(z|c)$ are Gaussian distributions, so the formula is:
% \begin{equation}
\begin{align}
    %   h &= h_c \oplus h_r \nonumber\\
       h_q = &\mathrm{Encoder}([c;r]) \nonumber \\ 
       y = &\mathrm{Linear}(h_q)\nonumber \\ 
       h_p = &\mathrm{Encoder_c}(c) 
    %   \nonumber\\
    %   \mu^{'}, \sigma^{'} &= Linear(h_p) %\nonumber\\
\end{align}
% \begin{align}
%     %   h &= h_c \oplus h_r \nonumber\\
%       h_q &= Enc_{Bert}([c;r]) \nonumber\\
%     %   \mu, \sigma &= Linear(h_q)  \nonumber\\
%       y &= Linear(h_q) \nonumber\\
%       h_p &= Enc_{Bert}(c) 
%     %   \nonumber\\
%     %   \mu^{'}, \sigma^{'} &= Linear(h_p) %\nonumber\\
% \end{align}
% \end{equation}
where $h_q$ is the representation of the pair containing the context $c$ and the reference $r$, which is used to learn the aggregated posterior distribution $q(z|c,r)$ of CMN. 
In contrast to EMS~\cite{chan_enhancing_2021}, which does not model the order information of the context-reference pair, we add the segment embedding, which allows CMN to distinguish the order of the context and the reference. 
Finally, $y$ is the output of the NSP task, and $h_p$ is the representation of context, which is utilised to learn the prior distribution $p(z|c)$.
% $h_q$ has two utilities: judge the relation between context and response and produce aggregated posterior distribution $q(z|c,r)$ of CVAE. Lastly, $y$ is the output of the NSP task and $h_p$ is the representation of context, which is utilised to learn the prior distribution $p(z|c)$.

To address the one-to-many issue in open-domain dialogue evaluation, we introduce the NSP objective into the CVAEs' training process to enhance our model's discriminability of feasible responses given contexts. 
%\textcolor{red}{mismatched context-response sentence pair}. 
Introducing NSP leads to two different scenarios when training CMN. Specifically for the NSP task, we randomly replace the reference with the response from other conversations in the training set with a 0.5 probability, where the resulting context-response pairs are regarded as the negative samples. Likewise, the contexts paired with the original references are the positive samples. 

\noindent\textbf{Training with positive samples.}~~When training with the positive training samples, we add the NSP loss to the CVAEs' loss, where the NSP loss can be viewed as additional regularisation, which enables the CVAEs model to capture the sequential dependencies between the context and response during the training stage. Therefore, the posterior and prior distributions and the sampled latent variables from them can contain rich sentence order and pair matching information.
%provide a restriction that makes the distribution can include order information. 
%When the input of the encoder is a positive sample, the NSP loss is regarded as an additional loss to CVAE's loss. Otherwise, the model is trained as a normal CVAE. as the latter will only approximate the former when the input sentence pair is matched during the training process.
% \begin{equation}
    \begin{align}
           &\mathcal{L}_{\text{train}}=E_{q(z|c, r)}[\log p(r|c, z)]\nonumber\\&-K L(q(z|c,r)||p(z|c)) - \log _{e} p(y=1) %\log _{10} 3   
    \end{align}
% \end{equation}
where $E$ is the expectation, and $y=1$ represents the positive samples and $y=0$ represents the negative ones. 
% necessity of NSP, limitation of p(z|c)

\noindent\textbf{Training with negative samples.}~~When training with the negative samples, we exclude the KL divergence loss of CVAEs, as it is undesired to optimise the  prior of negative examples $q(z|c, r_{neg})$ to be close to the posterior in this case.
%did not want the latent space include such a response which is not the real response for the context.
 \begin{equation}
    %\begin{align}
        \mathcal{L}_{\text{train}}=E_{p(z|c)}[\log p(r|c, z)] - \log_{e}p(y=0)
%    \end{align}
 \end{equation}
%Introducing the Segment Embeddings of the NSP task enables the CVAE model to learn which sentence is conversational context and which one is the response, which, therefore, could enhance the information of the prior and posterior distribution of our model and enables the latent variables sampled from them to contain the sequential information of sentences.

% When the context and response sentence pair is a positive sample, the loss of CVAE during training phase is shown as following:


%discriminate mismatched pair
%Incorporating the NSP task loss function as a restriction to the traditional CVAE enables the model to filter out the mismatched context and response pair by randomly replacing the input reference. Therefore the posterior distribution will carry more precise latent response information, and so does the prior distribution, as the latter will only be forced to approximate the former when the input reference is unchanged. In other words, the context-reference pair is matched in the training set during the training process. Then the latent variables sampled from them can contain more precise feasible latent response information in the further mutual information calculation procedure.
%sentence order


\subsection{Evaluation Stage}

In the evaluation stage, we learn to score a response candidate by calculating its MI w.r.t. the conversation context $c$ and the reference $r$ in the latent space obtained in the training stage of CMN. 
%In the evaluation stage, we learn to judge the quality of the generated response candidate $x$ by calculating its semantic dependence of context $c$ and reference $r$. 
% Specifically, we feed conversational context $c$ and ground-truth reference pair $r$, and context $c$ and generated response $x$ pair to the CVAE model to get the posterior probabilities $q(z|c, r)$ and $q(z|c, x)$, respectively.

One challenge is that it is intractable to calculate  MI directly in our case as we only have access to the samples instead of the underlying distributions. 
To tackle this challenge, we employ InfoNCE, a contrastive learning method based on Noise Contrastive Estimation (NCE)~\cite{Gutmann2012NoiseContrastiveEO,logeswaran_content_2018} to  calculate the lower bound of MI between the latent variables of the two posterior probabilities $q(z|c, r)$ and $q(z|c, x)$ and prior probability $p(z|c)$ (see Figure~\ref{fig: Model} for illustration). Formally, the lower bound of MI is given as 
\begin{align}
\small
%\hspace{-100mm}
    & I(x,r) \geq {E}_{(x, r)}[F(x, r)]+\log_{e}(N-1)\nonumber\\
    &-E_x[\log_{e} \frac{1}{N-1} \sum_{r_{j} \in R_{neg}} e^{F(x,  r_{j})}] 
\label{InfoNCE}
\end{align}
where $x$ is the response candidate, $r$ is the ground-truth reference in the dataset, $r_{j}$ represents the negative response sample from the negative set $R_{neg}$, which is the reference from other conversation turns in the datasets, and $N$ is the number of negative samples. 

As the underlying posterior distributions are unknown, we first sample from each posterior probability to obtain the latent variables $z_1$ and $z_2$, which contain the context-reference and the context-response sentence pairs information, respectively. %After approximating the posterior probabilities with sampled latent variables, 
 %We extend its application in open dialogue evaluation field, to our best known, which is the first attempt to apply InfoNCE in dialogue evaluation field.
The sampling method mentioned above and functions $F(x, c)$, $F(x_j, c)$ in Eq.~\ref{InfoNCE} are defined as follows:
\begin{align} %^\intercal 
    F&(x, r)=z_1 \cdot z_2 \nonumber\\ %\indent 
    &z_1 \sim q(z|c, r) \nonumber\\ %\indent  
    &z_2 \sim q(z|c, x)\nonumber\\
    F&(r_j, x)=z_1' \cdot z_2  \nonumber\\ %\indent
    &z_1' \sim q(z|c, r_j) 
\label{Sample}
\end{align}
% \end{equation}
where $z_1$ and $z_2$ represent the positive latent variable samples while $z_1'$ represents the negative latent samples from the corresponding posterior distributions; $\cdot$ represents the dot product operation.
We can estimate the MI between response $x$ and reference $r$, $I(x,r)$, and the MI between context $c$ and response $x$, $I(c,x)$ according to Eq.~\ref{InfoNCE} and Eq.~\ref{Sample}.

%Specifically, we calculate the lower bound of MI of the generated references to the reference and to its context, respectively.
%Firstly, similar to other reference-based evaluation metrics, we measure the similarity between reference $r$ and generated response $x$ by estimating their MI via InfoNCE in the smooth latent space produced by the CVAE model. 
%Specifically,  we use the trained CVAE model in the first stage and feed conversational context $c$ and ground-truth reference pair $r$, context $c$ and generated response $x$ pair to the first encoder of it twice to acquire the posterior probabilities $q(z|c, r)$ and $q(z|c, x)$, respectively. 
%While calculating mutual information is challenging as we typically only have access to samples instead of the underlying distributions. In this situation, 
%We utilise InfoNCE to calculate the lower bound of MI between latent variables from two posterior probabilities. 

% to measure the semantic similarity between sentences. The MI can provide theoretical guarantee and comprehensive sentence semantic information.  

%The formula for using InfoNCE to compute the lower bound of mutual information of response candidate and gold reference is shown as follows:
 

% mutual information




% \begin{normalsize}
% \begin{align}
% %\hspace{-100mm}
%     I(x,r) \geq {E}_{(x, r)}[F(x, r)] &\nonumber\\
%     -E_x[\log_{e} \frac{1}{N-1} \sum_{r_{j} \in R_{neg}} &e^{F(x, r_{j})}+\log_{e}(N-1)]  
% \label{InfoNCE}
% \end{align}
% \end{normalsize}


% \begin{scriptsize}
% \begin{gather}
% %公式
%     & I(x,r) \geq {E}_{(x, r)}[F(x, r)]\nonumber\\
%     &-E_x[\log_{e} \frac{1}{N-1} \sum_{r_{j} \in R_{neg}} e^{F(x,  r_{j})}+\log_{e}(N-1)] 
% %公式
% \end{gather}
% \end{scriptsize}





%advantage of InfoNCE
% From Eq.~\ref{InfoNCE}, 
% The goal of utilizing InfoNCE to calculate the lower bound of mutual information between response and reference or response and context, is analogous to training the response candidate to discriminate which reference or context relate well to it. 
% Specifically, in Eq.8, function $F(x, r)$ is designed as the dot product format of two latent variables $z_1$ and $z_2$ sampled from the posterior probability, which contain the semantic information of context and reference pair and context and response candidate pair, respectively. By conducting dot product, the semantic similarity between the response candidate $x$ and the reference $r$, which is regarded as positive instance, can be calculated. Similarly, function $F(x, r_j)$ use the dot product to compute the semantic similarity of response candidate $x$ and the reference $r_j$ as well but $r_j$ is the reference from other conversation turns and is regarded as negative sample during computing. Therefore, by computing these two semantic similarities with positive and negative reference instances, the response candidate can be enabled to learn which sentence is semantically related well to it.


When calculating the final score for a candidate response, we also consider the NSP probability of the response candidate $x$ given conversational context $c$, in addition to the two MI values. 
The rationale behind this is that InfoNCE might have difficulty in measuring the semantic similarity of the response candidate $x$ and the reference $r$ when they are distant in semantics. The NSP probability serves as a natural weighting, allowing the model to focus more on $I(c,x)$, hence improving our method's robustness. 
When feeding the context-response pair to the trained CVAEs in the evaluation stage, the NSP probability $g$ can be calculated according to the following formula:
\begin{equation}
    g=\sigma(\mathrm{Linear}(\mathrm{Encoder}([c;x])))
\end{equation}
where $\sigma$ is the activation function, and $g$ is the probability that response $x$ is predicted as the next sentence of context $c$. 
%The NSP prediction probability $g$  ranges from 0 to 1, with 
A higher value of $g$ means that the degree of dependence between context $c$ and response candidate $x$ is higher, and vice versa. 

%NSP score
% In addition, to mitigate the shortcoming of InfoNCE: it is difficult to measure the semantic similarity of response candidate $x$ and reference $r$ when the two sentences are far away in semantics. 

%In the training phase, we introduce the NSP task and add the loss as the additional loss when the input sentence pair is a positive instance, which can be regarded as a regularisation of the CVAE's loss and enable the model to discriminate negative samples and recognise sentence order. 


%combination method
Finally, we score a response candidate $x$ with Eq.~\ref{eq:final_score}, representing the degree of how well the response candidate relates to the context. %to , which is used to compare with human annotations.
\begin{equation}
    \text{Score} = g * I(c,x) + I(x,r)
    \label{eq:final_score}
\end{equation}
% The $g$ is the NSP prediction probability, which ranges from 0 to 1, the closer to 1, the degree of dependence between context $c$ and response candidate $x$ is higher. 
Here $I(x,c)$ represents the semantic dependence of the context and the response candidate. Thus using $g$ to multiply $I(c,x)$ controls the amount of information flowing from $I(c,x)$. Moreover, we also consider the semantic dependence of the response candidate and the reference based on their MI, i.e., $I(x,r)$. %When computing the final score introducing both the MI score and NSP probability at the same time,  %these two Such a combination mechanism can consider 
Essentially, the relationship between $x$ and $c$, and that  between $x$ and $r$ can be considered simultaneously via Eq.~\ref{eq:final_score}, and the one-to-many problem can be handled directly. %To evaluate the effectiveness of the NSP score, we will also compute the final matching score by adding two types of MI, $I(c,x)$ and $I(x, r)$, directly.

\section{Experiment}
%\subsection{Datasets}
\noindent\textbf{Datasets.}~~To evaluate the effectiveness of our proposed automatic evaluation metric, we conduct experiments on two open dialogue datasets. 
The \textbf{PersonaChat} dataset~\cite{Zhang2018PersonalizingDA} is a large persona-conditioned chit-chat style dialogue dataset which consists of 10,907 multi-turn dialogue sessions. The \textbf{DailyDialog} dataset~\cite{Li2017DailyDialogAM} is another widely-used large collection of human-human dialogues, consisting of 13,118 multi-turn dialogue sessions. 

% Human-annotated Dataset. We collect the
% human-annotated datasets from Amazon Mechanical Turk and obtain two human-annotated datasets which consist of 750 context-response pairs in the
% persona-chat dataset and 800 ones in the dailydialog dataset, respectively. Following Zhao et al.(2020), the generated references come from several
% classical dialogue models, i,e., Seq2Seq (Sutskeveret al., 2014), Seq2Seq with Attention (Serban et al., 2016), HRED (Serban et al., 2017), VHRED (Ser-
% ban et al., 2016), GPT-2 (Wolf et al., 2019).

%\subsection{Baselines}
\noindent\textbf{Baselines.}~~We choose the following two kinds of evaluation metrics as baseline methods:

\noindent\textbf{Reference-Based Metrics.}~~For the reference-based metrics, we use BLEU~\cite{papineni_bleu_2002}, ROUGE~\cite{lin_rouge_2004}, METEOR~\cite{banerjee_meteor_2005}, Embedding-Average~\cite{Wieting2016TowardsUP}, Vector-Extrema~\cite{Forgues2014BootstrappingDS}, Greedy-Matching~\cite{Rus2012ACO}, BERTScore~\cite{Zhang2020BERTScoreET}, and BLEURT~\cite{Sellam2020BLEURTLR}, which have been widely used in generative dialogue systems.

\noindent\textbf{Reference-free Metrics.}~~For the reference-free metrics, we compare with two learning-based methods RUBER~\cite{Tao2018RUBERAU} and MAUDE~\cite{Sinha2020LearningAU}. Note that we are not able to compare with EMS~\cite{chan_enhancing_2021}, as their code is unavailable. It is also infeasible to re-implement their approach due to the lack of sufficient implementation details in the paper\footnote{We have contacted the authors of the paper regarding code and some implementation details, but have no response at all.}. 
%However, because of the ambiguity of the method description and  , and the code is not available as well, we cannot reproduce it, therefore it is not considered as a baseline.

% \noindent\textbf{reference-free Metrics.}~~We utilize BLEU score to measure n-grams overlaps between response reference and generated response. Speciﬁcally, we follow the conventional setting in Sinhaet al. (2020) and use the multibleu.
% \noindent\textbf{ROUGE.}~~ROUGE is the most popular metric in the text summarization task. There, we report the f1 score of Rouge-{1,2,3,L} and Rouge-L identiﬁes the longest common subsequence between the generated and reference to better account for sentence-level structure when computing word
% overlap.

% \noindent\textbf{METEOR.}~~The METEOR is designed as an improvement on BLEU using a harmonic mean of precision and recall, as well as stemming and synonyms. 

% \noindent\textbf{Embedding Metrics.}~~ Embedding Metrics compute the similarity between the embeddings representations of generated results and reference. The used embeddings come from glove6. In particular, we calculate three metrics: 1) Average, cosine similarity between the averaged word embedding in the two sentences ; 2) Extrema, cosine similarity between the largest extreme values among the word embeddings in the two sentences; 3) Greedy, i.e., greedily matching words in two sentences based on the cosine similarities, and the total scores are then averaged across all words.

% \noindent\textbf{BERTScore.}~~BERTScore uses a strong pre-trained language model to greedily match each word in a reference response with one word in the generated response. By doing so, it computes the recall of the generated sequence. BERTScore was shown to have strong system-level and segment-level correlation with human judgment on several machine translation tasks.

% \noindent\textbf{BLEURT.}~~BLEURT is based on the BERTScore and ﬁnetuned on human judgments after pretraining on large-scale synthetic data with multiple automatic metrics as supervision signals. BLEURT has shown its strong correlation with human judgment on machine translation tasks.

% \noindent\textbf{RUBER.}~~RUBER is an unsupervised automatic evaluation metric that considering the similarity of the generated response with conversational context and response reference.

% \noindent\textbf{MAUDE.}~~MAUDE proposed an unreferenced automated evaluation metric that uses large-scale PLMs to extract hidden representations of dialogue sentences, and leverages the temporal transitions that exist between them.

% \noindent\textbf{EMS.}~~EMS utilized smooth latent space to compete the semantic similarity between context $x$ and response $x$. 


\subsection{Setup} \label{Settings}

We use BERT~\cite{Devlin2019BERTPO} and GPT-2~\cite{Wolf2019TransferTransfoAT} as the encoder and the decoder of our CVAE model, respectively. We set the dimension of the latent variable $z$ of CVAE to 32.
Following~\citet{zhao_designing_2020}, we generate response candidates based on the conversational context of the PersonaChat and DailyDialog datasets using several widely applied dialogue generation systems, including Seq2Seq~\cite{sutskever_sequence_2014}, HRED~\cite{serban_hierarchical_2016}, and GPT-2~\cite{Wolf2019TransferTransfoAT}. 
We then collected 82 and 56 samples from DailyDialog and PersonaChat datasets, respectively, where the sample references and generated responses are very close in semantics (denoted as the \textit{standard set}). We also collected another 200 samples from each dataset, whose responses are distant to the references in semantics (denoted as the \textit{diversity set}), resulting in 508 samples\footnote{The sample number difference between the standard and diverse sets is mainly due to that there are much less generated responses which are very similar to the references.} in total for our experiment. 
The collection process is manual. 
%involves using our evaluation scores (based on Eq.~\ref{eq:final_score}) to pre-filtering samples, followed by manual inspections. 
We also ensure sure that the final set contains a balanced mixture of samples generated by different systems (i.e., Seq2Seq, HRED, and GPT-2).
%The standard of collecting sentence pairs is that the meaning expressed by context is clear and unambiguous.

\subsection{Further analysis of the diverse set}

To further validate that our diverse set indeed contains the reference and the generated response pairs whose semantics are very different (i.e., well suited for testing the one-to-many scenario), we conduct two different types of semantic analysis: the surface form word overlap and the embedding-based semantic similarity.
%, to fully demonstrate the effectiveness of our evaluation method in solving the one-to-many problem.

%Although the long-standing one-to-many nature of open-domain dialogue is a huge challenge for evaluation metrics, there has been insufficient experimental analysis. 

We use BLEU-1 to measure the surface form word overlap, where a lower BLEU-1 score can indicate a lower word repetition rate between the generated response and reference. %selected for human annotation
%the word repetition rate between the response candidate and reference needs to be low to ensure the diversity of responses. 
%We use BLEU-1 score to measure the word overlap rate. The lower BLEU-1 score indicates the lower word repetition rate between generated response and reference selected for human annotation.
The averaged BLEU-1 scores of the samples from the diverse set (200 samples for each dataset) are 0.12 (DailyDialog) and 0.08 (PersonaChat), respectively, indicating that the word repetition rates between the response candidates and the gold-standard references are low.
% While both Pearson and Spearman coefficients obtained by our method are superior, outperforming most baselines, showing that our method can solve the one-to-many problem. 

For embedding-based semantic similarity, we use BERTScore, where the resulting averaged scores are 0.23 (DailyDialog) and 0.27 (PersonaChat), respectively. This result also indicates that the reference and the response candidate are quite semantically different.%we argue that some response candidates are similar to corresponding references in semantics, though their word overlap rates are low. In this case, 
% In addition, we visualise the selected references from datasets and their corresponding response candidates by T-SNE clustering to demonstrate the data distributions in the semantic space. 
Furthermore, from Figure~\ref{fig:label} (c) and (d), we can observe two clear clusters representing response candidates and references, which again demonstrates the semantic difference between the references and responses. In summary, we can conclude that the diverse set is a good fit for testing the one-to-many scenario.  

\begin{figure*}[ht]
\small
\centering 
    \subfigure[]{
% 	\includegraphics[width = 0.33\textwidth]{dd_similar.png}}
	\includegraphics[width = 0.38\textwidth]{dd_similar.png}}
% 	\hfill
	\subfigure[]{
% 	\includegraphics[width = 0.33\textwidth]{personachat_similar.png}}
	\includegraphics[width = 0.38\textwidth]{personachat_similar.png}}
% 	\hfill
	\subfigure[]{
% 	\includegraphics[width = 0.33\textwidth]{dd_diversity.png}}
	\includegraphics[width = 0.38\textwidth]{dd_diversity.png}}
% 	\hfill
	\subfigure[]{
% 	\includegraphics[width = 0.33\textwidth]{personachat_diversity.png}}
	\includegraphics[width = 0.38\textwidth]{personachat_diversity.png}}
\caption{T-SNE visualisation of the sentence representation of references and generated responses. (a) and (b) for the \textit{standard set}, and (c) and (d) for the \textit{diverse set}.}
\label{fig:label}
\end{figure*}

%table1
\begin{table*}[h]
\centering
\begin{threeparttable}[b]
\small
\begin{tabular}{lcc|cc}
             \toprule
              & \multicolumn{2}{c|}{DailyDialog}                                                          & \multicolumn{2}{c}{PersonaChat}     \\ \midrule
Metrics       & Pearson's $\rho$                            & Spearman's $\tau$                           & Pearson's $\rho$ & Spearman's $\tau$ \\ \midrule
%dd pc

BLEU-1         & 0.0280 (0.8025)                             & -0.1378 (0.2169)                              & 0.0567 (0.6770)             & 0.0282 (0.8362)              \\
BLEU-2         & 0.0129 (0.9081)                             & -0.1320 (0.237)                            & -0.0235 (0.8621)             & -0.0678 (0.6192)                \\
BLEU-3         & -0.0378 (0.7362)                             & -0.1508 (0.1761)                             & -0.0239 (0.8602)                 & -0.0539 (0.6927)               \\
BLEU-4         & 0.0134 (0.9047)                            & -0.0914 (0.4139)                            & -0.0896 (0.5101)                  & -0.0906 (0.5060)                \\ \midrule

ROUGE-1        & 0.0623 (0.5784)                            & -0.1415 (0.2048)                           & 0.0460 (0.7360)                  & 0.1224 (0.3682)                 \\
ROUGE-2        & -0.0248 (0.8249)                           &  -0.1538 (0.1677)                          & 0.0408 (0.7654)               & 0.0548 (0.6880)             \\
ROUGE-L             & 0.0473 (0.6728)                             & -0.1432 (0.1992)                            & 0.0251 (0.8534)              & 0.1177 (0.3871)                 \\ \midrule

METEOR        &    0.1184 (0.2895)                          &   0.1630 (0.1435)                          &   -0.0826 (0.5448)              &  -0.0800 (0.5576)            \\  \midrule
Embedding      &                                             &                                             &                  &    
        \\
Extrema        &  0.2617 (0.0174)                         & -0.0238 (0.8313)                            & -0.3019 (0.0231)                & 0.1726 (0.2038)
    \\
Greedy        &  0.0850 (0.4433)                         &  0.1631 (0.1435)                      & -0.1070 (0.4320)                 & 0.013 (0.9231)
    \\
Average        & -0.0070 (0.9433)                           & 0.0435 (0.6972)                            & -0.0461 (0.7350)                & 0.0212 (0.8762)
    \\ \midrule
BERTScore     & 0.096 (0.3881)            & -0.1688 (0.1292)                 & 0.1296 (0.3403)                  & 0.1681 (0.2150)                \\
BLEURT        & 0.1968 (0.0701)                            & -0.1239 (0.2672)                            & 0.0251 (0.8531)                & 0.0392 (0.7732)                 \\
\midrule
RUBER         & 0.1240 (0.2668)                  & 0.1482 (0.1837)                           &  0.0022 (0.9871)           & -0.1006 (0.4603)                  \\
MAUDE         & -0.1255 (0.2613)                             & 0.0458 (0.6827)                            & 0.2201 (0.1035)                 & 0.2723 (0.0423)                 \\
\midrule

%\tnote{1}
% Ours(w/o NSP ) & -0.1830 (0.0992)                             & -0.2264 (0.0401)                           & 0.1316 (0.3334)                 & 0.0989 (0.4686)                 \\ %\tnote{2}
Ours(w/o NSP) & 0.2844 (0.0090)                             & 0.1545 (0.1655)                            & 0.3214 (0.0152)                 & \textbf{0.3622 (0.0067)}                  \\
Ours(w/o MI)  &     0.2505 (0.0232)                             & 0.0432 (0.6994)                           &  0.1721 (0.2045)                & 0.0352 (0.7961)                  \\

Ours  & \textbf{0.3388 (0.0024)}                  & \textbf{0.2369 (0.0320)}            & \textbf{0.3386 (0.0106)}              & 0.3585 (0.0063)                   \\
\bottomrule

\end{tabular}
\end{threeparttable}
\caption{Pearson and Spearman correlations with human judgements on the standard set.}
\label{tab:similar_correlation}
\end{table*}

%table1 commented
% \begin{table*}[h]
% \centering
% \begin{threeparttable}[b]
% \small
% \begin{tabular}{lcc|cc}
%              \toprule
%               & \multicolumn{2}{c|}{DailyDialog}                                                          & \multicolumn{2}{c}{PersonaChat}     \\ \midrule
% Metrics       & Pearson's $\rho$                            & Spearman's $\tau$                           & Pearson's $\rho$ & Spearman's $\tau$ \\ \midrule
% %dd pc
% BLEU-1         & -0.2465 (0.0021)                             & -0.6188 (<0.001)                              & 0.0567 (0.6770)             & 0.0282 (0.8362)              \\
% BLEU-2         & -0.2020 (0.0680)                             & -0.5684 (<0.001)                             & -0.0235 (0.8621)             & -0.0678 (0.6192)                \\
% BLEU-3         & -0.2269 (0.0403)                             & -0.5289 (<0.001)                             & -0.0239 (0.8602)                 & -0.0539 (0.6927)               \\
% BLEU-4         & -0.1647 (0.1392)                             & -0.4259 (<0.001)                             & -0.0896 (0.5101)                  & -0.0906 (0.5060)                \\ \midrule

% ROUGE-1        & -0.0260 (0.8161)                            & -0.2291 (0.0384)                           & 0.0460 (0.7360)                  & 0.1224 (0.3682)                 \\
% ROUGE-2        & -0.0880 (0.4133)                           & -0.2733 (0.0128)                           & 0.0408 (0.7654)               & 0.0548 (0.6880)             \\
% ROUGE-L             & -0.0350 (0.748)                             & -0.2306 (0.0375)                            & 0.0251 (0.8534)              & 0.1177 (0.3871)                 \\ \midrule
% METEOR        &    0.1184 (0.2895)                          &   0.1630 (0.1435)                          &   -0.0826 (0.5448)              &  -0.0800 (0.5576)            \\  \midrule
% Embedding      &                                             &                                             &                  &    
%         \\
% Extrema        &  0.2617 (0.0174)                         & -0.0238 (0.8313)                            & -0.3019 (0.0231)                & 0.1726 (0.2038)
%     \\
% Greedy        &  0.0850 (0.4433)                         &  0.1631 (0.1435)                      & -0.1070 (0.4320)                 & 0.013 (0.9231)
%     \\
% Average        & -0.0070 (0.9433)                           & 0.0435 (0.6972)                            & -0.0461 (0.7350)                & 0.0212 (0.8762)
%     \\ \midrule
% BERTScore     & 0.096 (0.3881)            & -0.1688 (0.1292)                 & 0.1296 (0.3403)                  & 0.1681 (0.2150)                \\
% BLEURT        & 0.1968 (0.0701)                            & -0.1239 (0.2672)                            & 0.0251 (0.8531)                & 0.0392 (0.7732)                 \\
% \midrule
% RUBER         & 0.1240 (0.2668)                  & 0.1482 (0.1837)                           &  0.0022 (0.9871)           & -0.1006 (0.4603)                  \\
% MAUDE         & -0.1255 (0.2613)                             & 0.0458 (0.6827)                            & 0.2201 (0.1035)                 & 0.2723 (0.0423)                 \\
% \midrule

% %\tnote{1}
% % Ours(w/o NSP ) & -0.1830 (0.0992)                             & -0.2264 (0.0401)                           & 0.1316 (0.3334)                 & 0.0989 (0.4686)                 \\ %\tnote{2}
% Ours(w/o NSP) & 0.2844 (0.0090)                             & 0.1545 (0.1655)                            & 0.3214 (0.0152)                 & \textbf{0.3622 (0.0067)}                  \\
% Ours(w/o MI)  &     0.2505 (0.0232)                             & 0.0432 (0.6994)                           &  0.1721 (0.2045)                & 0.0352 (0.7961)                  \\

% Ours  & \textbf{0.3388 (0.0024)}                  & \textbf{0.2369 (0.0320)}            & \textbf{0.3386 (0.0106)}              & 0.3585 (0.0063)                   \\
% \bottomrule

% \end{tabular}
% \end{threeparttable}
% \caption{Pearson and Spearman correlations with human judgements on the standard set.}
% \label{tab:similar_correlation}
% \end{table*}

\subsection{Human evaluation settings}
Following the work of~\citet{Howcroft2020TwentyYO}, we set two human evaluation criteria: \textit{appropriateness} and \textit{coherence}, each of which is set on a 1-5 \textit{Likert} scale, with a higher scale indicating a better measure. Concretely, the criteria are defined as follows:
\noindent\textbf{Appropriateness}: The degree to which the generated response is conversationally related well to the given context.
\noindent\textbf{Coherence}: The degree to which the content/meaning of 
output is presented in a well-structured, logical and meaningful way. E.g. “\textit{Does the generated text accord with the correct logic?}”

%(from bad to good readability quality). 
We ask two human annotators to evaluate the context-response pair according to the above criteria, and average their scores to produce the final score. 
Both annotators hold at least a master's degree in Computer Science, and have full professional proficiency in English. During the human evaluation, the annotators are presented with the conversation context and generated responses from the 508 samples described above. 

% We also examined the inter-rater reliability. Following~\citet{lan_pone_2020}, it is computed by holding out the ratings of one rater at a time, calculating its correlation (i.e., Pearson and Spearman) with the other rater’s judgments, and finally averaging over all held-out correlation scores. 
We also examined the inter-rater reliability. Following~\citet{lan_pone_2020}, it is computed by holding out the ratings of one rater and calculating its correlation (i.e., Pearson and Spearman) with another rater’s judgment.
%In terms of the Inter-Annotator Agreement, we  follow~\citet{lan_pone_2020} to calculate the Pearson and Spearman correlations between two human annotators. 
%We first calculate the correlation for the diverse semantic samples
For the standard setting experiment, the Pearson’s $\rho$ and the Spearman’s $\tau$ are 0.69 and 0.64 for the DailyDialog, and 0.74 and 0.70 for PersonaChat, respectively.
For the one-to-many setting experiment, the Pearson’s $\rho$ and Spearman’s $\tau$ are 0.76 and 0.72 for DailyDialog, and 0.36 and 0.32 for PersonaChat, respectively.



%The inter-rater reliability results also support the strong performance of our proposed context coherence metric in that the correlation between the automatic metric and human evaluation was close to the inter-rater correlations.


\section{Results}
% We first produce response candidates on selected sentence pairs by generative models, such as Seq2Seq, GPT-2 and HRED. Therefore 
We conduct experiments to evaluate our model performance on the open-domain dialogue evaluation for two different scenarios. One is the common scenario where the generated responses are semantically very similar to the references (denoted as the \textit{standard setting}), and the other is the generated responses which are semantically distant to the references (denoted as the \textit{one-to-many setting}).  
% , but are contextually relevant to the context
%In this section, we evaluate each dataset by our proposed method and compare the results with baselines. In addition, as mentioned in \cref{Settings}, we selecte similar and diverse semantic samples from two datasets. To show the data distributions, we first calculate the representation of the reference and the generated response and demonstrate them with T-SNE in Figure~\ref{fig:label}, where the data points in (a) and (b) are for the similar semantic samples while that in (c) and (d) are for the diverse semantic ones. We will analyse it in the next section.


\begin{table*}
\centering
\begin{threeparttable}[b]
\small

\begin{tabular}{lcc|cc}
             \toprule
              & \multicolumn{2}{c|}{DailyDialog}                                                          & \multicolumn{2}{c}{PersonaChat}     \\ \midrule
Metrics       & Pearson's $\rho$                            & Spearman's $\tau$                           & Pearson's $\rho$ & Spearman's $\tau$ \\ \midrule
%BLEU          &                                             &                                             &                  &                   \\
BLEU-1        & 0.1993 (0.004)                             & 0.1821 (0.008)                             & -0.0967 (0.1880)                 &  -0.0846 (0.2499)                 \\
BLEU-2        & 0.1074 (0.125)                             & 0.1696 (0.015)                             &   -0.1168 (0.1113)               & -0.1119 (0.1272)                  \\
BLEU-3        & 0.0569 (0.417)                             & 0.1465 (0.035)                             &   -0.1200 (0.1019)                &  -0.1256 (0.0867)                 \\
BLEU-4        & 0.0317 (0.651)                             & 0.1363 (0.051)                             &   -0.1203 (0.1011)                &  -0.132 (0.0717)                 \\ \midrule
%ROUGE         &                                             &                                             &                  &                   \\
ROUGE-1        & 0.2718 (<0.0001)                             & 0.2605 (<0.0001)                            &  -0.0287 (0.6971)                 &  0.0587 (0.4249)                 \\
ROUGE-2        & 0.2334 (<0.0001)                            & 0.2321 (<0.0001)                           &   -0.0704 (0.3382)                & 0.0533 (0.4685)                  \\
ROUGE-L             & 0.2886 (<0.0001)                             & 0.2806 (<0.0001)                             &   -0.0319 (0.6650)               &  0.0579 (0.4312)                 \\ \midrule
METEOR        & 0.1831 (0.008)                             & 0.1646 (0.018)                             &        0.0976 (0.1837)          & 0.1056 (0.1502)             \\  \midrule
Embedding      &                                             &                                             &                  &    
        \\
Extrema        & -0.1290(0.064)                           & -0.1600(0.021)                             & -0.0471(0.521)                 & -0.0248(0.735) 
    \\
Greedy        & -0.0500(0.468)                           &  -0.1120(0.107)                            & 0.0006(0.9934)                 &0.0838(0.2539)
    \\
Average        & -0.1320(0.058)                           &  -0.1730(0.013)                            &  0.0120(0.870)                &-0.0256(0.727)
    \\ \midrule
BERTScore     & 0.4234 (<0.0001)                           & 0.4833 (<0.0001)                           & 0.0241(0.7431)                 & 0.0795(0.2790)                  \\
BLEURT        & 0.3021 (<0.0001)                            & 0.2759 (<0.0001)                            & 0.1283(0.0800)                 & 0.1863(0.0106)                   \\
\midrule
RUBER         & 0.1505 (0.0310)                           & 0.1279 (0.0670)                           & -0.1139 (0.1200)           &  -0.1094 (0.1350)                  \\
MAUDE         & 0.1365 (0.0508)                             & 0.2365 (<0.0001)                             &  0.2308 (0.0014)                &  \textbf{0.3281 (<0.0001)}                 \\
\midrule
% Ours(w/o NSP\tnote{1} ) & 0.0805 (0.250)                             & 0.1427 (0.041)                            &  0.0086 (0.9064)                & 0.0591 (0.4214)                  \\
% \tnote{2}
Ours(w/o NSP) & 0.1995 (0.004)                             & 0.3312 (<0.001)                            &  0.2961(0.0025)                & 0.2196 (0.0025)                  \\
Ours(w/o MI)  & \textbf{0.5104 (<0.0001)} & 0.4830 (<0.0001)                           & 0.2193(0.0025)                 &  0.1835(0.0117)                 \\

Ours         & 0.4942 (<0.0001)                           & \textbf{0.5177(<0.0001)} & \textbf{0.3246(<0.0001)}               &  0.3125(<0.0001)                   \\
\bottomrule

\end{tabular}
%  \begin{tablenotes}
%   \item [1] no NSP loss in Training Phase.
%   \item [2] NSP loss included in Training Phase but not in Evaluation Phase, which means $g$=1 in Eq.10
%  \end{tablenotes}
\end{threeparttable}
\caption{Pearson and Spearman correlations with human judgements on the diverse set.}

\label{tab:correlation}
\end{table*}

\subsection{Model evaluation in the standard setting}
%To validate the effectiveness of the MI part in our method in evaluating open-domain dialogue, 

As described in \S~\ref{Settings}, the \textit{standard set} contains samples from the DailyDialog and PersonaChat datasets,  whose references and generated responses are very close in semantics. 
%we select 82 and 56 similar semantic samples from the DailyDialog and the PersonaChat datasets, respectively. 
Figure~\ref{fig:label} (a) and (b) shows the T-SNE visualisation of the sentence representation of the references and generated responses from the set. 
It can be observed that the response candidates are similar to the references, where the corresponding data points are very close to each other or even overlapping, e.g., there are many overlapping points in Figure~\ref{fig:label} (a), resulting in an effect which seems to be more points in orange.  
%in semantics  data points for the references and the generated responses are close to each other. 

%\vspace{-mm}
We compare our model to the baselines in terms of how well the model produced evaluation scores correlate with human judgement scores. 
%each response candidate by our proposed method and compare the results that of baselines.
As shown in Table~\ref{tab:similar_correlation}, our CMN model achieves the best overall performance for both Pearson and Spearman correlations on both datasets, where RUBER and MAUDE appear to be the best performing baselines on the DailyDialog and PersonaChat datasets, respectively.
% DailyDialog dataset, the Pearson correlation is 0.3388, and the Spearman correlation is 0.2369. 
%DailyDialog dataset, with Pearson and Spearman correlation coefficients of 0.3388 and 0.2369, respectively.
%\textcolor{red}{
We also conducted ablation studies to evaluate the effectiveness of the MI (w/o NSP) and the NSP (w/o MI) components by excluding the other component when computing the final evaluation score.  
%only using the NSP probability in the evaluation phase .}
%by using these two parts to conduct experiments separately, which can be viewed as ablations of our proposed method. 
It can be observed that the performance of CMN with the MI component alone (i.e., w/o NSP) gives better performance than the model with the NSP component.   
This suggests that  MI is more effective than NSP in evaluating dialogues when the response candidates are similar to the references in semantics.



\subsection{Model evaluation in the one-to-many setting}
%\subsection{Performance on semantically diverse datasets} 

In another set of experiments, we evaluate our model performance in the one-to-many setting based on the \textit{diverse set}, in which the responses are distant from the references in semantics. 
%We conduct the experiments on 400 selected conversational context-reference pairs from DialyDialog and PersonaChat dialogue datasets (200 pairs each).

%diverse dataset
%It can be observed that traditional embedding based metrics perform the worst on both Pearson and Spearman correlations, suggesting poor correlation with human annotations. 
As shown in Table~\ref{tab:correlation}, Extrema, Greedy, and Average %achieve negative correlation or weak correlation with human annotation scores on both datasets.
achieve a negative or weakly positive correlation with human annotation scores on both datasets. This is a similar observation to that of \citet{Liu2016HowNT}, who also discovered that the embedding-based metrics weakly correlate with human judgements.
% N-gram based metrics perform better than traditional embedding based one. BLEU, ROUGE, and METEOR's correlations with human scores are less than 0.3 on both datasets. 
The word overlap metrics based on $n$-gram perform better than the above traditional embedding-based ones, with BLEU, ROUGE, and METEOR all having higher correlation than the embedding-based approaches.  
Nevertheless, these metrics still give relatively weak correlations for both datasets.  
%(e.g., BLEU achieves less than 0.2 correlations on the both datasets).

% BLEU scores drop less than 0.2 when the n-gram increases, though it is widely used in machine translation. Similar phenomena are obtained on ROUGE and METEOR, and both metrics give weak correlations on both datasets.

On the other hand, embedding-based metrics which use pre-trained models to represent sentences achieve much better results than the aforementioned baselines. For instance, BERTScore achieves more than 0.4 and BLEURT achieves close to 0.3 for both Pearson and Spearman correlations on DailyDialog, although there is some performance drop on PersonaChat.
%, which might be due to the fact that \textcolor{red}{[xx]}. 

As for reference-free metrics, the performances for RUBER and MAUDE are not as good as expected on the DailyDialog dataset. However, MAUDE performs the best on the PersonaChat dataset in terms of Spearman correlation (0.3281), which is slightly higher than our method. %The reason might be the different data distribution between the reference and the response candidate. We will analyse it in the following section.

In summary, our CMN model achieves the best overall performances on both datasets, giving the highest scores for both Pearson (0.5104) and Spearman (0.5177) correlations on DailyDialog, and the highest Pearson correlation on PersonaChat (0.3246). 
%We validate our method's performance by conducting ablation study. Specifically.
Our ablation studies also show that NSP is crucial in evaluating dialogues when there is a significant difference between references and responses in semantics. By introducing NSP, our model can effectively capture the contextual dependencies between the conversational context and generated responses, and thus can better handle the one-to-many issue in open-domain dialogue evaluation. 
%One may notice that our full model performs slightly worse than our model variant when excluding the MI component (i.e., w/o MI), this might be 

%response candidate by considering the relation to its conversational context and thus solve the one-to-many nature.

%In summary, the experimental results demonstrate that our method gives the best performance in terms of correlation with human annotator scores for both the DailyDialog and PersonaChat datasets, and both the standard and diverse settings.
% To demonstrate the effect of the data distribution between references and our 
%To demonstrate our method's superiority in dealing with the one-to-many problem, we conduct a semantic diversity analysis in the next section.

\begin{table}[h]
\small
\begin{tabular}{cccl}
\toprule
\multicolumn{1}{l}{\textbf{Context:}}   & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}How long will it take for my passport to be ready?\end{tabular}}                                      \\ \midrule
\multicolumn{1}{l}{\textbf{Reference:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}You will get it in a few weeks .\end{tabular}}                                                                                                             \\ \midrule
\multicolumn{1}{l}{\textbf{Generated:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}It's about 20 minutes.\end{tabular}}                        \\ \midrule
Human                          & BLEU                                               & MAUDE                                             & \multicolumn{1}{c}{RUBER}                                          \\ %\hline
5.0                            & 1.0                                              & 3.57                                             & \multicolumn{1}{c}{0.28}                                            \\ \hline
BERTScore                      & BLEURT                                             & Ours                                              &                                                                    \\ %\hline
1.69                          & 1.50                                              & 4.42                                              &                                                                    \\ \midrule[2pt]
\multicolumn{1}{l}{\textbf{Context:}}   & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}Are you writing a book now?\end{tabular}}                                                                                                                            \\ \hline
\multicolumn{1}{l}{\textbf{Reference:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}Yes, it's about a group of friends living in a foreign country, and all the strange experiences they have.\end{tabular}} \\ \hline
\multicolumn{1}{l}{\textbf{Generated:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}Yes, I'm very interested in it.\end{tabular}}                                                                                                                     \\ \midrule[1pt]
Human                          & BLEU                                               & MAUDE                                             & \multicolumn{1}{c}{RUBER}                                          \\ %\hline
4.66                           & 1.35                                               & 4.0                                               & \multicolumn{1}{c}{4.4}                                            \\ \hline
BERTScore                      & BLEURT                                             & Ours                                              &                                                                    \\ %\hline
1.47                           & 1.28                                               & 4.12                                              &                                                                    \\ \bottomrule
\end{tabular}
\caption{Samples from DailyDialog dataset.}
\label{tab:case study1}
\end{table}
\subsection{Case Studies}
For qualitative analysis, we show two cases of our experiment in Table~\ref{tab:case study1}. Each case shows the conversational context as well as the corresponding gold-standard reference and the generated response. We compare our evaluation score with five different baselines. To simplify the comparison, we normalise all scores to a range of 1-5 to be consistent with the Likert scale of human evaluation. Note that the normalisation is applied to the case study only, not conducted in the previous experiments.
In the first case, the generated response is relatively similar to the reference, whereas the reference and response are very different in the second case.  
For both cases, our CMN gives very similar scores to the human scores.  
%From these examples from the PersonaChat and the DailyDialog datasets, the matching score of our method correlated well with the human annotation score. 
More examples are provided in Appendix A.


% \begin{table}[H]
% \small
% \begin{tabular}{cccl}
% \toprule
% \multicolumn{1}{l}{\textbf{context:}}   & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}the market is fairly down right now , so the offer is a realistic one .\end{tabular}}                                      \\ \midrule
% \multicolumn{1}{l}{\textbf{reference:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}when will we know if they accept the offer?\end{tabular}}                                                                                                             \\ \midrule
% \multicolumn{1}{l}{\textbf{generated:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}good news. well, we 'll make thecemberment to get someouses for our new bought goods.\end{tabular}}                        \\ \midrule
% Human                          & BLEU                                               & MAUDE                                             & \multicolumn{1}{c}{RUBER}                                          \\ %\hline
% 4.0                            & 0.335                                              & 4.365                                             & \multicolumn{1}{c}{4.4}                                            \\ \hline
% BERTScore                      & BLEURT                                             & Ours                                              &                                                                    \\ %\hline
% 0.54                           & 1.88                                               & 3.70                                              &                                                                    \\ \midrule[2pt]
% \multicolumn{1}{l}{\textbf{context:}}   & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}are you writing a book now ?\end{tabular}}                                                                                                                            \\ \hline
% \multicolumn{1}{l}{\textbf{reference:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}yes , it 's about a group of friends living in a foreign country , and all the strange experiences they have\end{tabular}} \\ \hline
% \multicolumn{1}{l}{\textbf{generated:}} & \multicolumn{3}{l}{\begin{tabular}{p{5cm}}yes , i ' m very interested in it .\end{tabular}}                                                                                                                     \\ \midrule[1pt]
% Human                          & BLEU                                               & MAUDE                                             & \multicolumn{1}{c}{RUBER}                                          \\ %\hline
% 4.66                           & 1.35                                               & 4.0                                               & \multicolumn{1}{c}{4.4}                                            \\ \hline
% BERTScore                      & BLEURT                                             & Ours                                              &                                                                    \\ %\hline
% 1.47                           & 1.28                                               & 4.12                                              &                                                                    \\ \bottomrule
% \end{tabular}
% \caption{Samples from DailyDialog dataset}
% \label{tab:case study1}
% \end{table}



\section{Conclusions}

In this paper, we propose a novel learning-based automatic evaluation metric which can robustly evaluate the open-domain dialogue by augmenting the CVAEs with the NSP objective and employing the MI to model the semantic similarity of text in the latent space.  %To the best of our knowledge, it is the first attempt to extend the application of MI in the open-domain evaluation field.%We provide a detailed analysis of the effectiveness in dealing with one-to-many nature.
Experimental results on two open-domain dialogue datasets show that our CMN model outperforms a wide range of baseline methods in both Pearson and Spearman correlations with human annotation scores, and is superior in dealing with the one-to-many issue of the open-domain dialogue evaluation.
%In addition, we perform a detailed analysis of the effectiveness of our proposed method on both semantically diverse and similar sentence pairs and validate that our method is superior in dealing with the one-to-many nature of open-domain dialogue. 

\section*{Ethic Impact}

In this paper, we propose a new automatic evaluation metric CMN to evaluate the open-domain dialogue system. The positive impact of CMN is that it can deal with the one-to-many problem in the open-domain dialogue evaluation metrics. The negative impact lies in that the CMN may potentially give a high score to the rude and dirty responses in some extreme cases. So we need to examine the training datasets before training the CMN.

\section*{Limitations}

Although our proposed method performs well in evaluating the open-domain dialogue systems, it also has some limitations. Our method identifies the dependencies between context and response. However, according to \citet{Howcroft2020TwentyYO}, human-evaluated metrics can contain a variety of attributes whilst we only identify the large-scale dependencies of semantics and do not disentangle the texts into the attributes of human-evaluated metrics. In the future, we will conduct disentanglement studies to disentangle the text into various attributes to optimise our model and further improve the interpretability of text evaluation methods based on these disentangled attributes.
% \subsection{Appendices}

% Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.


% \section*{Acknowledgements}



% Entries for the entire Anthology, followed by custom entries
